Large-Scale Demonstration of Precise Demand Response Provided by Residential Heating Systems

Being able to adjust the demand of electricity can be an effective means for power system operators to compensate fluctuating renewable generation, to avoid grid congestion, and to cope with other contingencies. Electric heating and cooling systems of buildings can provide different demand response services because their electricity consumption is inherently flexible because of their thermal inertia. This paper reports on the results of a large-scale demand response demonstration involving a population of more than 300 residential buildings with heat pump installations. We show how the energetic behavior and flexibility of individual systems can be identified autonomously based only on energy meter data and outdoor air temperature measurements, and how the aggregate demand response potential of the population can be quantified. Various load reduction and rebound damping experiments illustrate the effectiveness of the approach: the load reductions can be predicted precisely and amount to 40-65% of the aggregate load, and the rebound can be damped efficiently.

==> estimateFlex.tex <==
%\addtolength{\textheight}{-11.5mm}
\section{ESTIMATION OF FLEXIBILITY}
\label{s:estimateFlex}
This section introduces a quantitative description of the energetic flexibility based on time-varying power and energy constraints. The proposed description adopts a discrete-time perspective. It captures the flexibility available over a planning horizon comprising $N$ time steps each of length $t_s$. The flexibility is described by the set of all power trajectories that satisfy the power and energy constraints of the system. Flexibility descriptions of this type serve as the basis for applications ranging from controlling energy systems \cite{Sundstroem2012,Trangbaek2012} to minimizing energy procurement costs \cite{Gonzalez2015,Mathieu2013} and providing ancillary services \cite{Hao2014}.

\subsection{Constraints on Power}
An estimate of the rated heating power has been derived in \sect\ref{ss:identRatedPower}. This value is to be interpreted as the average power the system will consume during a heating period. Thus, the power consumption $p_k$ of the heating system is restricted to
\begin{equation}
	p_k\in\{0,\,\pre\},\,k=0,\dots,N-1.
	\label{eq:powerConstr}
\end{equation} 

\subsection{Constraints on Energy}
As discussed in \sect\ref{s:sysModeling}, a domestic building and its heating system are modeled as a single energy buffer. The discrete-time version of the linearized energy dynamics \eqref{eq:approxEnergyDyn} is
\begin{equation}
	e_{k+1} = e_k + t_s\left(\bar{q}_c^k u_k-\bar{q}_l^k\right),\ k=0,\dots,N-1.
	\label{eq:dtEnergyDyn}
\end{equation}
The thermostat controller of the heating system keeps the energy level $e_k$ within the bounds ${[e_{\min},\,e_{\max}]}$ and thereby guarantees that comfort constraints are satisfied. The flexible portion $e_{\ts{flex}}$ of the building energy, \cf\fig\ref{fig:energyDynamics}, can be interpreted as the capacity of a battery with state of charge (SOC) ${x_k:=(e_k-e_{\min})/(e_{\max}-e_{\min})}$. From this definition follows that 
%\begin{align}
%	  0 & \leq x_k\leq 1,\,&k&=0,\dots,N-1\nonumber\\
%	 \Leftrightarrow\ e_{\min} & \leq e_k\leq e_{\max},\,&k&=1,\dots,N.
%	 \label{eq:energyConstr}
%\end{align}
\begin{equation}
	  0\leq x_k\leq 1\ \Leftrightarrow\ e_{\min}\leq e_k\leq e_{\max},\,k=0,\dots,N.
	 \label{eq:energyConstr}
\end{equation}
Substituting $e_k$ in \eqref{eq:dtEnergyDyn} by $x_k$ yields the SOC dynamics
\begin{equation*}
	x_{k+1} = x_k + t_s(\bar{r}_c^k u_k - \bar{r}_l^k),\ k=0,\dots,N-1,
	%\label{eq:socDynamics1}
\end{equation*}
which use the normalized average loss and charge rates $\bar{r}_l$ and $\bar{r}_c$. Their temperature dependency is captured by $\bar{r}_l(\bar{\theta}_{\ts{out}})$ and $\bar{r}_c(\bar{\theta}_{\ts{out}})$ captured by \eqref{eq:lossRateTempRel} and \eqref{eq:chargeRateTempRel}. To forecast the flexibility available, \eqref{eq:lossRateTempRel} and \eqref{eq:chargeRateTempRel} are used to predict the normalized rates based on forecasts of the outdoor air temperature. Let $\hat{\theta}_{\ts{out}}^k$ denote the average outdoor temperature forecast for the time interval ${[t_sk,\,t_s(k+1)]}$. Then, the estimate of $\bar{r}_c^k$ is $\bar{r}_c(\hat{\theta}_{\ts{out}}^k)$, and similarly for $\bar{r}_l^k$. Thus, predictions of the SOC are 
\begin{equation}
	\hat{x}_{k+1} = \hat{x}_{k} + t_s[\bar{r}_c(\hat{\theta}_{\ts{out}}^k)u_k -\bar{r}_l(\hat{\theta}_{\ts{out}}^k)].
	\label{eq:socDynamics}
\end{equation}
Applying \eqref{eq:socDynamics} at the current time $t_0$ requires an estimate of the initial SOC. It can be computed as follows:
\begin{equation*}
	\hat{x}_0 = 
	\begin{cases}
		1-\bar{r}_l(\bar{\theta}_{\ts{out}})[t_0-\hat{t}_{\ts{off}}(\ts{end})] &\mbox{if } \hat{t}_{\ts{off}}(\ts{end})>\hat{t}_{\ts{on}}(\ts{end})\\
		\bar{r}_c(\bar{\theta}_{\ts{out}})[t_0-\hat{t}_{\ts{on}}(\ts{end})] &\mbox{otherwise},
	\end{cases}
\end{equation*}
with $\bar{\theta}_{\ts{out}}$ being the average outdoor air temperature measured since the last switching action of the heating system.

%between the current time $t_0$ and the time of the last switching action:
%\begin{equation*}
%	\bar{\theta}_{\ts{amb}}= \ts{mean}(\theta_{\ts{amb}}(t)),\ t\in [t_{\ts{switch}},\,t_0],
%\end{equation*}
%where $t_{\ts{switch}}:=\max\{\hat{t}_{\ts{on}}(\ts{end}),\,\hat{t}_{\ts{off}}(\ts{end})\}$.

At every time step $k$, the input ${u_k\in\{0,\,1\}}$ can be chosen freely, subject to the constraint that the next SOC satisfies the energy constraints \eqref{eq:energyConstr}, \ie, ${x_{k+1}\in[0,1]}$. Let ${\hat{x}:=[\hat{x}_1,\dots,\hat{x}_N]\trans\in\R{N}}$, ${u:=[u_0,\dots,u_{N-1}]\trans\in\R{N}}$. The predicted SOC evolution $\hat{x}$, \cf\eqref{eq:socDynamics}, for a particular input trajectory $u$ can be written compactly as
\begin{equation}
	\hat{x}=\hat{x}_0\mathbf{1}+Bu-d,
	\label{eq:socLdDyn}
\end{equation}
with matrix ${B\in\R{N\times N}}$, whose $i^{\ts{th}}$ row is given as $$B_i=t_s[\bar{r}_c(\hat{\theta}_{\ts{out}}^0),\,\bar{r}_c(\hat{\theta}_{\ts{out}}^1),\,\dots,\bar{r}_c(\hat{\theta}_{\ts{out}}^{i-1}),\,0,\,\dots,0],$$
and vector $d\in\R{N}$, whose $i^{\ts{th}}$ element is given as $$d_i=t_s\left(\bar{r}_l(\hat{\theta}_{\ts{out}}^1)+\bar{r}_l(\hat{\theta}_{\ts{out}}^2)+\dots+\bar{r}_l(\hat{\theta}_{\ts{out}}^{i-1})\right).$$ A vector of ones of appropriate size is denoted by $\mathbf{1}$.
%\begin{equation*}
%	B = t_s\begin{bmatrix}
%	\bar{r}_c(\hat{\theta}_{\ts{amb}}^0) & 0 & \dots & 0\\
%	\bar{r}_c(\hat{\theta}_{\ts{amb}}^0) & \bar{r}_c(\hat{\theta}_{\ts{amb}}^1) & & \vdots\\
%	\vdots & & \ddots & 0\\
%	\bar{r}_c(\hat{\theta}_{\ts{amb}}^0) & \bar{r}_c(\hat{\theta}_{\ts{amb}}^1) & \dots & \bar{r}_c(\hat{\theta}_{\ts{amb}}^{N-1})
%	\end{bmatrix}\in\R{N\times N}
%\end{equation*}
%and vector
%\begin{equation*}
%	d = t_s\begin{bmatrix}
%		\bar{r}_l(\hat{\theta}_{\ts{amb}}^0)\\
%		\bar{r}_l(\hat{\theta}_{\ts{amb}}^0)+\bar{r}_l(\hat{\theta}_{\ts{amb}}^1)\\
%		\vdots\\
%		\bar{r}_l(\hat{\theta}_{\ts{amb}}^0)+\dots+\bar{r}_l(\hat{\theta}_{\ts{amb}}^{N-1})
%	\end{bmatrix}\in\R{N}.
%\end{equation*}

Using \eqref{eq:socLdDyn} and ${p_k=\pre u_k}$, the energy constraints \eqref{eq:energyConstr} can be reformulated as constraints on the power consumption $p$ of the heating system over a given planning horizon as
\begin{equation}
 	\begin{bmatrix}
 	B\\ -B
 	\end{bmatrix}
 	p \leq 
 	\pre\begin{bmatrix}
 		(1-\hat{x}_0)\mathbf{1}+d\\
 		\hat{x}_0\mathbf{1}-d
 	\end{bmatrix},
 	\label{eq:enConstrOnPower}
\end{equation}
where  ${p:=[p_0,\dots,p_{N-1}]\trans\in\R{N}}$. Inequalities \eqref{eq:enConstrOnPower} define a convex polytope in $\R{N}$ that contains all the power trajectories that are feasible with regard to the energy limits.

The power and energy constraints \eqref{eq:powerConstr} and \eqref{eq:enConstrOnPower} describe the set of power trajectories that the system can follow over a given planning horizon while meeting comfort constraints. This set is called the \emph{feasible set}. It represents a quantitative description of the energetic flexibility of the system over a finite planning horizon. Moreover, its formulation as a set makes it particularly convenient to use for control and optimization purposes.

\fig\ref{fig:flex} visualizes the energetic flexibility available over $12$ h with sampling time ${t_s=5}$ min. The initial SOC is ${x_0=0.75}$. For every time step, the maximum and the minimum possible cumulative energy have been computed. The shaded gray area between these lines is a measure of the flexibility because all feasible trajectories must lie in it. The flexibility of the system allows the heating to start immediately or to be deferred for at most $4$ time steps, see the inset. Also shown is the outdoor air temperature, which influences the flexibility available.

\begin{figure}[tb]
\setlength{\abovecaptionskip}{-5pt}
%\setlength{\belowcaptionskip}{-50pt}
\centering
\psfrag{xlabel}[Bc][Bc][1.3]{Time of day}
\psfrag{ylabel1}[Bc][Bc][1.3]{Cumulative energy [kWh]}
\psfrag{ylabel2}[Bc][Bc][1.3]{Outdoor air temperature [$\degc$]}
\psfrag{xlabelin}[Bc][Bc][1]{Time index $k$}
\psfrag{ylabelin}[Bc][Bc][1]{[kWh]}
\psfrag{emax}[Bc][Bc][1.3]{$\max$}
\psfrag{emin}[Bc][Bc][1.3]{$\min$}
\psfrag{theta}[Bc][Bc][1.3]{$\theta_{\ts{out}}$}
\resizebox{0.5\textwidth}{!}{
\includegraphics[]{flex.eps}
}
\caption{Minimum and maximum cumulative energy trajectories over $12$ h with sampling time ${t_s=5}$ min and ${x_0=0.75}$. The inset plot shows a detail view of the first $6$ time slots. The flexibility of the system allows the heating to start immediately or to be deferred for at most $4$ time steps. The loss and charge rates that determine the shape of the energy trajectories depend on the outdoor air temperature (dashed line) via \eqref{eq:lossRateTempRel} and \eqref{eq:chargeRateTempRel}.}
\label{fig:flex}
\end{figure}
